AdLER: Adversarial Training with Label Error Rectification for One-Shot Medical Image Segmentation

Accurate automatic segmentation of medical images typically requires large datasets with high-quality annotations, making it less applicable in clinical settings due to limited training data. One-shot segmentation based on learned transformations (OSSLT) has shown promise when labeled data is extremely limited, typically including unsupervised deformable registration, data augmentation with learned registration, and segmentation learned from augmented data. However, current one-shot segmentation methods are challenged by limited data diversity during augmentation, and potential label errors caused by imperfect registration. To address these issues, we propose a novel one-shot medical image segmentation method with adversarial training and label error rectification (AdLER), with the aim of improving the diversity of generated data and correcting label errors to enhance segmentation performance. Specifically, we implement a novel dual consistency constraint to ensure anatomy-aligned registration that lessens registration errors. Furthermore, we develop an adversarial training strategy to augment the atlas image, which ensures both generation diversity and segmentation robustness. We also propose to rectify potential label errors in the augmented atlas images by estimating segmentation uncertainty, which can compensate for the imperfect nature of deformable registration and improve segmentation authenticity. Experiments on the CANDI and ABIDE datasets demonstrate that the proposed AdLER outperforms previous state-of-the-art methods by 0.7% (CANDI), 3.6% (ABIDE "seen"), and 4.9% (ABIDE "unseen") in segmentation based on Dice scores, respectively. The source code will be available at https://github.com/hsiangyuzhao/AdLER.

==> data/abide.tex <==
\begin{table}[h]
\centering
\caption{Performance comparison of different OSSLT methods on ABIDE benchmark \cite{ding2021modeling}.}
\label{table:abide}
\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{ccccccc}
\toprule
\multirow{3}{*}{\textbf{Method}}     & \multicolumn{6}{c}{\textbf{Metric} (\textbf{DSC \% $\uparrow$})}                        \\ 
                                     \cline{2-7}
                                     & \multicolumn{3}{c}{ABIDE Seen}      & \multicolumn{3}{c}{ABIDE Uneen}   \\
                                     \cline{2-7}
                                     & Mean±Std & Min                     & Max  & Mean±Std   & Min   & Max   \\ 
\midrule
DataAug \cite{zhao2019data}          & 69.6 ± 9.0 & 33.1                    & 82.5 & 64.3 ± 9.9   & 32.3  & 79.6  \\
LT-Net \cite{wang2020lt}             & 71.3 ± 9.2 & 39.7                    & 80.4 & 66.1 ± 9.4   & 35.0  & 77.2  \\
VAEAug \cite{ding2021modeling}       & 76.7 ± 7.4 & 53.2                    & 86.5 & 74.8 ± 6.6   & 54.1  & 83.3  \\
BRBS \cite{he2022learning}           & 77.5 ± 8.6 & 54.4                    & 87.6 & 74.5 ± 7.1   & 53.8  & 83.6  \\
\midrule
Ours                                 & \textbf{81.1 ± 7.9} & \textbf{55.2} & \textbf{89.5} & \textbf{79.4 ± 3.3} & \textbf{70.4} & \textbf{86.1} \\
\bottomrule
\end{tabular}
}
\end{table}

==> data/candi.tex <==
\begin{table}
\centering
\caption{Performance comparison of different OSSLT methods on CANDI dataset.}
\label{table:candi}
\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{4mm}{
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Metric} (\textbf{DSC \% $\uparrow$})}   \\ 
\cline{2-4} 
                                     & Mean±Std        & Min         & Max          \\ 
\midrule
DataAug \cite{zhao2019data}          & 80.4 ± 4.3        & 73.8        & 84.0         \\
LT-Net \cite{wang2020lt}             & 82.3 ± 2.5        & 75.6        & 84.2         \\
VAEAug \cite{ding2021modeling}       & 85.1 ± 1.9        & 80.2        & 87.8         \\
BRBS \cite{he2022learning} \tablefootnote{Minimal and maximum segmentation DSC are not reported in the original paper. We obtain the results based on our reproduction.}           & 85.7 ± 1.0        & 81.3        & 87.5         \\
\midrule
Ours                                 & \textbf{86.4 ± 1.5} & \textbf{83.3} & \textbf{88.6}  \\
\bottomrule
\end{tabular}
}
\end{table}
% \begin{table}
% \centering
% \caption{Performance comparison of different OSSLT methods on CANDI dataset.}
% \label{table:candi}
% \begin{threeparttable}
% \renewcommand\arraystretch{1.1}
% \setlength{\tabcolsep}{4mm}{
% \begin{tabular}{cccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Metric} (\textbf{DSC \% $\uparrow$})}   \\ 
% \cline{2-4} 
%                                      & Mean±Std        & Min         & Max          \\ 
% \midrule
% DataAug \cite{zhao2019data}          & 80.4 ± 4.3        & 73.8        & 84.0         \\
% LT-Net \cite{wang2020lt}             & 82.3 ± 2.5        & 75.6        & 84.2         \\
% VAEAug \cite{ding2021modeling}       & 85.1 ± 1.9        & 80.2        & 87.8         \\
% BRBS \cite{he2022learning} \tnote{*} & 85.7 ± 1.0        & 81.3        & 87.5         \\
% \midrule
% Ours                                 & \textbf{86.4±1.5} & \textbf{83.3} & \textbf{88.6}  \\
% \bottomrule
% \end{tabular}
% }
% \begin{tablenotes}\footnotesize
% \item[*] Minimal and maximum segmentation DSC are not reported in the original paper. We obtain the results based on our reproduction.
% \end{tablenotes}
% \end{threeparttable}
% \end{table}

==> data/pseudo_code.tex <==
\begin{algorithm}[h]
\caption{Pseudo-code for training}
\label{sec:algorithm}

\KwIn{Registration network $\mathcal{R}$; adversarial network $\mathcal{G}$; segmentation network $\mathcal{S}$}
\KwOut{Trained segmentation network $\mathcal{S}$ for inference}
\KwData{Atlas $(x_A,y_A)$; Unlabeled dataset $\mathcal{D}_{U}$}
Set the target training iteration number $N_{all}$\;

\For{i {\rm in} range($N_{all}$)}{
Sample reference images $x_s$ and $x_a$ from $\mathcal{D}_{U}$\;

\tcp{first train registration}
\While{$\mathcal{R}$.{\rm requires\_grad}=\textit{True}}{
Train the registration $\mathcal{R}$ and get the loss $\mathcal{L}_{reg}$\;
Optimize the registration: $\min\limits_{\mathcal{R}} \mathcal{L}_{reg}$ \;
}

Freeze the registration: $\mathcal{R}$.requires\_grad=\textit{False}\;
Generate transformations: \begin{tabular}[t]{@{}l}$\phi=\mathcal{R}(x_A, x_s)$;\\ $\psi=\mathcal{R}(x_A, x_a)$ \end{tabular} \\
Augment the atlas: $x_g=(x_A+\psi) \circ \phi$;$y_g=y_A \circ \phi$\;

\tcp{train augmentation}
\While{$\mathcal{G}$.{\rm requires\_grad}=\textit{True}}{
Sample the transformation: \begin{tabular}[t]{@{}l}$\alpha,\beta=\mathcal{G}(x_g)$;\\ $\phi_{a}=\alpha \times \phi$;\\  $\psi_{a}=\psi+\beta \times \bar{\psi}$
\end{tabular} \\
Adversarial augment: $x_{ag}=(x_A+\psi_{a}) \circ \phi_{a}$\;
Segmentation: $\hat{y}_{g}=\mathcal{S}(x_g)$, \ $\hat{y}_{ag}=\mathcal{S}(x_{ag})$\;
% \tcc{adversarial training, maximize difference}
% Optimize the augmentation: $\max\limits_{\mathcal{G}} \mathcal{L}_{adv}(\hat{y}_{g}, \hat{y}_{ag})$\;
Optimize the augmentation: $\max\limits_{\mathcal{G}} \mathcal{L}_{adv}$\;
}
Freeze the augmentation: $\mathcal{G}$.requires\_grad=\textit{False}\;

\tcp{train segmentation}
\While{$\mathcal{S}$.{\rm requires\_grad}=\textit{True}}{
% \tcc{adversarial training, sample again, minimize difference}
Sample the transformation: \begin{tabular}[t]{@{}l}$\alpha',\beta'=\mathcal{G}(x_g)$;\\ $\phi_{a}'=\alpha' \times \phi$;\\  $\psi_{a}'=\psi+\beta' \times \bar{\psi}$
\end{tabular} \\
Adversarial augment: $x_{ag}'=(x_A+\psi_{a}') \circ \phi_{a}'$\;
Segmentation: $\hat{y}_{g}=\mathcal{S}(x_g)$, \ $\hat{y}_{ag}'=\mathcal{S}(x_{ag}')$\;
% \tcp{label error rectification}
Rectified segmentation: $\mathcal{L}_{seg}=\mathcal{L}_{str}+\mathcal{L}_{rec}$\;
% Optimize the segmentation: $\min\limits_{\mathcal{S}} (\mathcal{L}_{adv}(\hat{y}_{g}, \hat{y}_{ag}')+\mathcal{L}_{seg}$)\;
% \tcc{minimize both adversarial loss and rectified loss}
Optimize the segmentation: $\min\limits_{\mathcal{S}} (\mathcal{L}_{adv}+\mathcal{L}_{seg}$)\;
}
Freeze the segmentation: $\mathcal{S}$.requires\_grad=\textit{False}\;
Unfreeze the registration: $\mathcal{R}$.requires\_grad=\textit{True}\;
}
\end{algorithm}
